Hermes Attack: Steal DNN Models with Lossless Inference Accuracy

Deep Neural Networks (DNNs) models become one of the most valuable enterprise assets due to their critical roles in all aspects of applications. With the trend of privatization deployment of DNN models, the data leakage of the DNN models is becoming increasingly serious and widespread. All existing model-extraction attacks can only leak parts of targeted DNN models with low accuracy or high overhead. In this paper, we first identify a new attack surface -- unencrypted PCIe traffic, to leak DNN models. Based on this new attack surface, we propose a novel model-extraction attack, namely Hermes Attack, which is the first attack to fully steal the whole victim DNN model. The stolen DNN models have the same hyper-parameters, parameters, and semantically identical architecture as the original ones. It is challenging due to the closed-source CUDA runtime, driver, and GPU internals, as well as the undocumented data structures and the loss of some critical semantics in the PCIe traffic. Additionally, there are millions of PCIe packets with numerous noises and chaos orders. Our Hermes Attack addresses these issues by huge reverse engineering efforts and reliable semantic reconstruction, as well as skillful packet selection and order correction. We implement a prototype of the Hermes Attack, and evaluate two sequential DNN models (i.e., MINIST and VGG) and one consequential DNN model (i.e., ResNet) on three NVIDIA GPU platforms, i.e., NVIDIA Geforce GT 730, NVIDIA Geforce GTX 1080 Ti, and NVIDIA Geforce RTX 2080 Ti. The evaluation results indicate that our scheme is able to efficiently and completely reconstruct ALL of them with making inferences on any one image. Evaluated with Cifar10 test dataset that contains 10,000 images, the experiment results show that the stolen models have the same inference accuracy as the original ones (i.e., lossless inference accuracy).

==> backup.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Layers}                        & \textbf{Input Shape} & \textbf{Output Shape} & \textbf{\# Parameters} & \textbf{Hyper-Parameters}                                                                                             & \textbf{Kernels}                                                                                                                                                                                                                                                                                                                    \\ \hline
Convolution 2D              & (28,28,1)   & (26,26,32)  & 320           & \begin{tabular}[c]{@{}c@{}}Kernel Size: (3,3)\\ Filters: 32\\ Strides: (1,1)\\ Use\_Bias: True\\ AF: Relu \end{tabular} & \begin{tabular}[c]{@{}c@{}}tensorflow::functor::ShuffleInTensor3Simple()\\ cudnn::detail::implicit\_convolve\_sgemm()\\ im2col4d\_kernel()\\ fft2d\_r2c\_32x32()\\ tensorflow::BiasNCHWKernel()\\ Eigen::internal::scalar\_max\_op()\end{tabular} \\ \hline
Convolution 2D              & (26,26,32)  & (24,24,64)  & 18496         & \begin{tabular}[c]{@{}c@{}}Kernel Size: (3,3)\\ Filters: 64 \\ Strides: (1,1)\\ Use\_Bias: True\\ AF: Relu \end{tabular} & \begin{tabular}[c]{@{}c@{}}tensorflow::functor::ShuffleInTensor3Simple()\\ cudnn::detail::implicit\_convolve\_sgemm()\\ im2col4d\_kernel()\\ fft2d\_r2c\_32x32()\\ tensorflow::BiasNCHWKernel()\\ Eigen::internal::scalar\_max\_op()\end{tabular} \\ \hline
Maxpooling 2D   & (24,24,64)  & (8,8,64)    & \textbackslash{}             & Pool Size: (2,2)                                                                                            & cudnn::detail::pooling\_fw\_4d\_kernel                                                                                                                                                                                                                                                                                     \\ \hline
Dropout         & (8,8,64)    & (8,8,64)    & \textbackslash{}             & 0.25                                                                                                        & \textbackslash{}                                                                                                                                                                                                                                                                                                           \\ \hline
Flatten         & (8,8,64)    & 4096        & \textbackslash{}             & \textbackslash{}                                                                                            & \begin{tabular}[c]{@{}c@{}}SwapDimension1And2InTensor3UsingTiles()\\ tensorflow::functor::BlockReduceKernel()\end{tabular}                                                                                                                                                                                                 \\ \hline
Dense                     & 4096        & 128         & 524416        & \begin{tabular}[c]{@{}c@{}}Units: 128\\ Use\_Bias: True\\ AF: Relu\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}gemv2N\_kernel\_val()\\ tensorflow::BiasNHWCKernel()\\Eigen::internal::scalar\_max\_op()\end{tabular}                                                                                                                                                                                                                               \\ \hline
Dropout        & 128         & 128         & \textbackslash{}            & 0.5                                                                                                         & \textbackslash{}                                                                                                                                                                                                                                                                                                           \\ \hline
Dense                  & 128         & 10          & 1290          & \begin{tabular}[c]{@{}c@{}}Units: 10\\ Use\_Bias:True\\ AF: Softmax\end{tabular}                                          & \begin{tabular}[c]{@{}c@{}}gemv2N\_kernel\_val()\\ tensorflow::BiasNHWCKernel()\\softmax\_op\_gpu\_cu\_compute\_70()\end{tabular}                                                                                                                                                                                                                               \\ \hline
\end{tabular}
}
\caption{\hush{??} \textbf{The Original Model.} This table comprises the model architecture, number of parameters, hyper-parameters as well as executing kernels of the original model. AF in the \textbf{Hyper-Parameters} column stands for \emph{activation function}. The \textbf{Kernels} column lists the part of the involved kernels of each layer. 
}

\label{tbl:victim}
\end{table*}





\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Layers}         & \textbf{Input Shape} & \textbf{Output Shape} & \textbf{\# Parameters}    & \textbf{Hyper-Parameters}                                                                                             & \textbf{Primary Kernels}                                                                                                                           \\ \hline
Convolution 2D & (28,28,1)   & (26,26,32)  & 320              & \begin{tabular}[c]{@{}c@{}}Kernel Size: (3,3)\\ Filters: 32\\ Strides: (1,1)\\ Use\_Bias: True\\AF: Relu\end{tabular} & \begin{tabular}[c]{@{}c@{}}tensorflow::functor::ShuffleInTensor3Simple()\\ cudnn::detail::implicit\_convolve\_sgemm()\end{tabular} \\ \hline

Convolution 2D & (26,26,32)  & (24,24,64)  & 18496            & \begin{tabular}[c]{@{}c@{}}Kernel Size: (3,3)\\ Filters: 64 \\ Strides: (1,1)\\ Use\_Bias: True\\AF: Relu\end{tabular} & \begin{tabular}[c]{@{}c@{}}tensorflow::functor::ShuffleInTensor3Simple()\\ cudnn::detail::implicit\_convolve\_sgemm()\end{tabular} \\ \hline

Maxpooling 2D  & (24,24,64)  & (8,8,64)    & \textbackslash{}               & Pool Size: (2,2)                                                                                            & cudnn::detail::pooling\_fw\_4d\_kernel()                                                                                           \\ \hline
Flatten        & (8,8,64)    & 4096        & \textbackslash{}                & \textbackslash{}                                                                                            & tensorflow::functor::BlockReduceKernel()                                                                                           \\ \hline
Dense          & 4096        & 128         & 524416           & \begin{tabular}[c]{@{}c@{}}Units: 128\\ Use\_Bias: True\\AF: Relu\end{tabular}                                        & gemv2N\_kernel\_val()                                                                                                              \\ \hline

Dense          & 128         & 10          & 1290             & \begin{tabular}[c]{@{}c@{}}Units: 10\\ Use\_Bias:True\\AF: Softmax\end{tabular}                                          & gemv2N\_kernel\_val()                                                                                                              \\ \hline

\end{tabular}
}
\caption{\hush{??}\textbf{The Generated Model.} This table comprises the model architecture, number of parameters, hyper-parameters as well as examined primary kernels of the generated model. AF in the 
\textbf{Hyper-Parameters} 
column stands for \emph{activation function}. 
The \textbf{Primary Kernels} 
Column lists the kernels used to identify the layer type. Compared to the original model (in Table. \ref{tbl:victim}), the generated model has identical parameters, hyper-parameters, and architecture. The elimination of dropout layer is attributed to its quiescence in the inference procedure.}
\label{tbl:generatedmodel}
\end{table*}

==> cam_ready.tex <==
1. Name: Adversarial attack is not accurate (Section 6)

“Adversarial attack” is strange -- all attacks are adversarial. So, in Section 6, “Adversarial Attack” should be changed to “Adversarial Examples” as all the works discussed there are about adversarial examples (I assume). Also, reference [2] is data poisoning attack (training time), not attacks for generating adversarial examples (test time). Also, in the same section, when introducing black-box attacks, it might be better to cite well-known and peer-reviewed black-box attack papers.


2. Threat model: More threat models other than AI model privatization deployment environment. (autonomous driving, - )
   attack environment (AI privatization, autonomous driving, inference as a service), not only PCIe bus, other bus (e.g., USB) are also possible.
5. How to handle large models, and again, name issue.  (add more points, Algorithm etc.)
as a side note, the title "super large models" feels informal


8: Hermes (https://en.wikipedia.org/wiki/Hermes)
9. references (1) format, line break (2) page align, better fill entire page

10 Fig. -> Figure, and Table./Tab. -> Table etc. Sec. -> Section 


3.1. Vitim model: The accuracy of our mnist model is low, which may be not practical. (Has been mentioned twice) (argue point: not related with accuracy)
3.2. Consider more activation functions ().
3.3 approximation/compressed NN (citations, intro/scenario/related work)


6: Section 3.4 improve, from the logic flow perspective (polish)

7: pictures (enlarge) and more related works (more details) proofread all of the related works and make the related works accurate

{Also, reference [2] is data poisoning attack (training time), not attacks for generating adversarial examples (test time). I suggest authors proofread all of the related works and make the related works accurate. Also, in the same section, when introducing black-box attacks, it might be better to cite well-known and peer-reviewed black-box attack papers.}

11 name of Section 5.1 (Super Large DNN Models) Need a formal description.
larger, deeper, giant, large-size


==> response.tex <==
We thank the reviewers for their thorough comments.

1: threat model
This attack model is practical in the DNN-model privatization deployment environment. In fact, privatization deployment is becoming a big market in China and US, and model-extraction attacks are also a huge challenge for AI companies. For example, company A has a private high-quality DNN model for live-face authentication, and it would like to sell this DNN model to other companies with a license fee, e.g., million dollars per year. In this privatization deployment scenario, company A (the model owner) allows company B to use the DNN model but has the motivation to protect its confidentiality, while company B has the physical access to its own machines and also has the motivation to steal the DNN model to save the license fee for the coming years.  Here company A usually protects its model with existing software-hardening and model-protection techniques on the host side, e.g., with secure boot, full disk encryption, runtime access control, and root privilege restrictions, etc. In addition, all existing model extraction works are NOT able to reconstruct the whole DNN model. Thus, at this point, people still have the illusion that the model is safe (or at least the leakage is acceptable). However, in this paper, we identify that the PCIe bus connecting the host and the GPU/AI-accelerator is a new attack surface and allows an adversary to FULLY reconstruct the WHOLE DNN model. We believe this attack technique can also work to other similar scenarios, such as a smartphone with NPU. We will revise the introduction and the threat model sections to clarify the practicality of the threat model in the new version.


2: Experiments
(testing on blackbox model; white-box model: Comparison between extracted model and original model; testing on complex large-size model)

We did black-box testing in our experiment. Specifically, in this experiment, we have no prior knowledge of the victim model. Thus, we adopt inference accuracy as the test metrics and evaluate it using 10,000 images. The experiment results indicate the accuracy for these 10,000 images is the exact the same. 

We also conducted a white-box experiment for a detailed comparison between the original model and the generated model. Specifically, we compared the hyper-parameters, parameters and model architecture between the original model and generated model. All hyper-parameters and parameters of the generated model are 100 \% identical with the original model. Note that
DNN inference procedure does not use any dropout layers and thus the generated model does not have such layers.

The model-extraction technique should be the same to handle large-size models. At this point, we have not tested it since the snooping device currently we are using has limited buffer size. Due to a large amount of noise in the traffic and the metadata of PCIe packets, the intercepted packets would quickly fill the whole buffer, resulting in the loss of the following packets. We will try to update our hardware or use other approaches to overcome this limitation in the future. 

About our experiment setup, the victim model is distinct from our while-box training models.  Each training model only includes a few selected layers. We will clarify the experiment setup and enrich the evaluation in the new version.

3: Comparison to existing works
We carefully compared our work with existing extraction attacks and use below table to display the major differences (will add it in the new version):

|              Work              |  Information Source  |    Method    |              |      Results     |            |
|:------------------------------:|:--------------------:|:------------:|:------------:|:----------------:|:----------:|
|                                |                      |              | Architecture | Hyper-Parameters | Parameters |
|    Xing Hu, et al. 2019 [18]   |   Access Pattern     |    Predict   |       ✔      |         X        |      X     |
| Yan, Mengjia, et al. 2018 [44] |         Cache        |    Search    |       X      |         ✔       |      X    |
|  Weizhe Hua, et al. 2018 [19]  |      Accelerator     | Search,Infer |       ✔      |         X        |      P     |
|   Yun Xiang et al. 2019 [41]   |         Power        |    Predict   |       ✔     |         ✔       |    X   |
| Vasisht Duddu et al. 2018 [14] |        Timing        |    Search    |       ✔      |         X        |      X     |
|  Binghui Wang et al. 2019 [38] |      Parameters      |     Infer    |       X    |         ✔        |      X  |
| Seong Joon Oh et al. 2018 [28] |       Querying       |     Infer    |       P      |         P       |      X     |
|            **Our Work**            |       **PCIe Bus**       |     **Infer**    |       ✔      |         ✔        |      ✔ |
In this table,  ✔ stands for fully recover, P stands for partial recover, X means can't recover.




\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Work} & \multirow{2}{*}{Information Source} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Results} \\ \cline{4-6}
 &  &  & Architecture & Hyper-Parameters & Parameters \\ \hline
Xing Hu, et al. 2019 {[}18{]} &  Access Pattern & Predict & 
\checkmark & \times  &\times  \\ \hline
Yan, Mengjia, et al. 2018 {[}44{]} & Cache & Search & \times  & \checkmark & \times \\ \hline 
Weizhe Hua, et al. 2018 {[}19{]} & Accelerator & Search,Infer & \checkmark & \times  & P \\ \hline
Yun Xiang et al. 2019 {[}41{]} & Power & Predict & \checkmark & \checkmark & \times \\ \hline
Vasisht Duddu et al. 2018 {[}14{]} & Timing & Search & \checkmark & \times & \times  \\ \hline

Binghui Wang et al. 2019 {[}38{]} & Parameters & Infer & \times & \checkmark & \times \\ \hline
Seong Joon Oh et al. 2018 {[}28{]} & Querying & Infer & P & P & \times \\ \hline 
\textbf{Our work} & \textbf{PCIe Bus} & \textbf{Infer} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} \\ \hline
\end{tabular}
}
\caption{\checkmark stands for fully recover, P stands for partial recover, $\times$ means can't recover.}
\end{table*}

4: writing
Thanks for the valuable suggestions. We will significantly improve our writing in the camera-ready version.

==> revisionletter.tex <==
% \begin{appendices}
% \label{sec:appendix}
% \section{Revision Letter}
% The entire paper is rewritten for
% clarity based on reviewer feedback and now includes a practical threat model (Sec.~\ref{sec:intro} and ~\ref{sec:overview}), further experiments (Sec.~\ref{evaluation}), as well as comparisons with existing related works (Sec.~\ref{relatedwork}). 


% \vspace{1mm}\noindent\textbf{Threat Model.}
% We have revised the introduction and the threat model sections (Sec.~\ref{sec:intro} and Section~\ref{sec:overview}) to clarify the practicality of the threat model. The threat model is practical because the attackers have both strong motivation (i.e., saving money) and sufficient ability (i.e., physical access and snoop PCIe traffic) to steal AI models from PCIe bus. We discussed the generalization of our attack to other similar scenarios, such as a different GPU platform or a smartphone with NPU (Sec.~\ref{generalization}).

% \vspace{1mm}\noindent\textbf{Experiments.}
% We comprehensively improve our experiment and evaluation.
% Specifically, in the previous submission we evaluated our attack with the MNIST model, which is a small sequential model. To show the effectiveness of our attack, we add more experiments on two more popular DNN models - VGG and ResNet. The VGG model is a sequential model with a very large number of parameters, and ResNet is a typical non-sequential model. All these experiments are black-box attacks. For each model, we also evaluate the inference accuracy (i.e., the same accuracy with original one), reconstruction efficiency, and the detailed architecture and hyper-parameters comparisons. All detailed descriptions are in Sec.~\ref{evaluation}. 
% %(testing on blackbox model; white-box model: Comparison between extracted model and original model; testing on complex large-size model)

% \vspace{1mm}\noindent\textbf{Comparisons with Existing Works.}
% We carefully compared our work with existing model extraction attacks, and used Sec.~\ref{relatedwork} and Table~\ref{tbl:relatedwork} to display the differences. The comparison results indicate that our \name is the only attack that can fully reconstruct the DNN model (including architecture, hyper-parameters, and parameters).


% \vspace{1mm}\noindent\textbf{Writing.}
% We have rewritten the whole paper, improved the writing, and enhanced the readability.

% \end{appendices}
